Spiking Nonlinear Opinion Dynamics (S-NOD) for Agile Decision-Making

We present, analyze, and illustrate a first-of-its-kind model of two-dimensional excitable (spiking) dynamics for decision-making over two options. The model, Spiking Nonlinear Opinion Dynamics (S-NOD), provides superior agility, characterized by fast, flexible, and adaptive response to rapid and unpredictable changes in context, environment, or information received about available options. S-NOD derives through the introduction of a single extra term to the previously presented Nonlinear Opinion Dynamics (NOD) for fast and flexible multi-agent decision-making behavior. The extra term is inspired by the fast-positive, slow-negative mixed-feedback structure of excitable systems. The agile behaviors brought about by the new excitable nature of decision-making driven by S-NOD are analyzed in a general setting and illustrated in an application to multi-robot navigation around human movers.

==> notation.tex <==
\newcommand{\reals}{\mathbb{R}}
\newcommand{\naturals}{\mathbb{N}} 
\newcommand{\rationals}{\mathbb{Q}}
\newcommand{\integers}{\mathbbb{Z}}
\newcommand{\compl}{\mathsf{c}}
\newcommand{\bdry}{{\partial}}
\newcommand{\symm}{\mathbb{S}}

\theoremstyle{remark}% default
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{lemma}{Lemma}
\newtheorem{remark}{Remark}
\newtheorem{proposition}{Proposition}
\newtheorem{assumption}{Assumption}
\newtheorem{definition}{Definition}
\renewcommand\qedsymbol{$\blacksquare$}

\newcommand{\AF}[1]{{\color{blue} (AF: #1)}}
\newcommand{\NL}[1]{{\color{magenta} (NL: #1)}}
\newcommand{\CC}[1]{{\color{ForestGreen} (CC: #1)}}
\newcommand{\IX}[1]{{\color{Melon} (IX: #1)}}

\newcommand{\squeezeup}{\vspace{-2.5mm}}
